Contrastive Mixture of Posteriors for Counterfactual Inference, Data Integration and Fairness

Learning meaningful representations of data that can address challenges such as batch effect correction and counterfactual inference is a central problem in many domains including computational biology. Adopting a Conditional VAE framework, we show that marginal independence between the representation and a condition variable plays a key role in both of these challenges. We propose the Contrastive Mixture of Posteriors (CoMP) method that uses a novel misalignment penalty defined in terms of mixtures of the variational posteriors to enforce this independence in latent space. We show that CoMP has attractive theoretical properties compared to previous approaches, and we prove counterfactual identifiability of CoMP under additional assumptions. We demonstrate state-of-the-art performance on a set of challenging tasks including aligning human tumour samples with cancer cell-lines, predicting transcriptome-level perturbation responses, and batch correction on single-cell RNA sequencing data. We also find parallels to fair representation learning and demonstrate that CoMP is competitive on a common task in the field.

==> relwork.tex <==
\section{Related Work}
\label{sec:relwork}
The problem of batch correction in data integration has been addressed using linear \cite{Johnson2007AdjustingBE, Leek2007CapturingHI} and nonlinear methods \cite{Haghverdi2018BatchEI, warren2020global} that perform transformations of the original feature space. In both cases, the goal is to transform the feature space so that information related to the scientific question of interest is retained while dependence on the batch (or nuisance covariate) is reduced. Methods based on representation learning attempt to learn a low-dimensional representation, $\z=q(\x)$, which is independent of nuisance factors while also being a faithful representation of the original data \cite{louizos2015variational, lopez2018deep, lopez2018information, lotfollahi2019conditional, martens2020neural}. Of these, the work that is most similar to ours are the VFAE \cite{louizos2015variational}, in which the authors introduce an MMD \cite{gretton2012kernel} penalty to encourage the marginal distributions of $\z$ under different values of $c$ to be close, and the trVAE \cite{lotfollahi2019conditional}, where the MMD penalty is applied to the output of the first layer of the decoder, rather than to $\z$ directly. 
Representation learning algorithms for counterfactual inference have been shown to benefit from a penalty enforcing distributional similarity between the representations of the treated and untreated samples \cite{Johnson2007AdjustingBE}. 
Elsewhere, authors have applied the variational autoencoder to inference on causal graphs \cite{louizos2017causal, Kim2020CounterfactualFW, Pfohl19CounterFactual}.

